Robust recovery for stochastic block models

We develop an efficient algorithm for weak recovery in a robust version of the stochastic block model. The algorithm matches the statistical guarantees of the best known algorithms for the vanilla version of the stochastic block model. In this sense, our results show that there is no price of robustness in the stochastic block model. Our work is heavily inspired by recent work of Banks, Mohanty, and Raghavendra (SODA 2021) that provided an efficient algorithm for the corresponding distinguishing problem. Our algorithm and its analysis significantly depart from previous ones for robust recovery. A key challenge is the peculiar optimization landscape underlying our algorithm: The planted partition may be far from optimal in the sense that completely unrelated solutions could achieve the same objective value. This phenomenon is related to the push-out effect at the BBP phase transition for PCA. To the best of our knowledge, our algorithm is the first to achieve robust recovery in the presence of such a push-out effect in a non-asymptotic setting. Our algorithm is an instantiation of a framework based on convex optimization (related to but distinct from sum-of-squares), which may be useful for other robust matrix estimation problems. A by-product of our analysis is a general technique that boosts the probability of success (over the randomness of the input) of an arbitrary robust weak-recovery algorithm from constant (or slowly vanishing) probability to exponentially high probability.

==> content/boosting-explanation.tex <==
\subsection{Boosting the probability of success of the algorithm}\label{sec:techniques}

%The approach described in \cref{sec:techniques} yields an algorithm that weakly recovers the communities vector  with constant probability. It turns out that we can exploit robustness to argue that, indeed, we can recover $\mathbf{x}$ with high probability.

%In fact, we will prove a very general boosting argument. We will show that as long as the probability of success of an arbitrary robust weak-recovery algorithm is not too small --- namely, greater than $e^{-n^{\frac{1}{4}}}$ --- then by paying a negligible price in the robustness and correlation guarantees of weak-recovery, we can boost the probability of success to at least $1-e^{-n^{\frac{1}{4}}}$.


%The boosting argument relies on a concentration of measure inequality known as the \emph{blowing-up lemma}, and which is widely used in information theory to prove strong converse results. Roughly speaking, the blowing-up lemma states that if $\mathbf{y}_1,\ldots,\mathbf{y}_N$ are $N$ independent random variables taking values in a finite set, and $\mathcal{E}_N$ is an event on $\mathbf{y}_1,\ldots,\mathbf{y}_N$ whose probability does not decay exponentially, i.e., $\displaystyle\lim_{N\to\infty}\frac{1}{N}\log\frac{1}{\mathbb{P}[\mathcal{E}_N]}=0$, then there exists $\ell_N=o(N)$ such that if we add to $\mathcal{E}_N$ all the strings $(y_1,\ldots,y_N)$ that are at a Hamming distance of at most $\ell_N=o(N)$ from $\mathcal{E}_N$, the probability of the obtained event becomes $1-o(1)$. 
%Since our algorithm is robust to a linear number of adversarial changes, then by paying a negligible (sublinear) price in the robustness and correlation guarantees, we can use the blowing-up to boost the probability of success of the algorithm to $1-o(1)$.




The approach described in \cref{sec:techniques} yields an algorithm that weakly recovers the communities vector  with constant probability. The main reason for this is that we only showed that the required structural inequalities hold with constant probability.\footnote{In fact, it is possible to prove that the structural inequalities hold with high probability without invoking the boosting argument. However, the needed calculations are more complicated. In any case, the boosting argument has the advantage of achieving exponentially high probability.} It turns out, however, that we can exploit robustness to argue that, indeed, we can weakly recover $\mathbf{x}$ with high probability.

The boosting argument relies on a concentration of measure inequality known as the \emph{blowing-up lemma} (see e.g., \cite{AhlswedeEtAlBlowingUp, MartonBlowingUp1, MartonBlowingUp2, ConcentrationOfMeasureRaginskySason}), and which is widely used in information theory to prove strong converse results\footnote{A strong converse result in information theory typically has the following form: If the rate of a code is above the capacity of a channel, then the probability of error of the code goes to 1 as the blocklength becomes large.}. Roughly speaking, the blowing-up lemma states that if $\mathbf{y}_1,\ldots,\mathbf{y}_N$ are $N$ independent random variables taking values in a finite set, and $\mathcal{E}_N$ is an event on $\mathbf{y}_1,\ldots,\mathbf{y}_N$ whose probability does not decay exponentially in $N$, i.e., $\displaystyle\lim_{N\to\infty}\frac{1}{N}\log\frac{1}{\mathbb{P}[\mathcal{E}_N]}=0$, then there exists $\ell_N=o(N)$ such that, if we "inflate" $\mathcal{E}_N$ by adding all the strings $(y_1,\ldots,y_N)$ that are at a Hamming distance of at most $\ell_N=o(N)$ from $\mathcal{E}_N$, then the probability of the obtained event becomes $1-o(1)$.

In our context of interest, this means that we do not need to directly show that our graph $\mathbf{G}\sim \sbm$ satisfies the desired structural inequalities (such as \cref{eq:informal-separation}). It suffices that \textit{some} graph $\tilde{G}\in N_{o(1)}(\mathbf{G})$ satisfies them. Since our algorithm is robust to a constant fraction $\rho$ of adversarial changes, and since $N_{\rho - o(1)}(\mathbf{G})\subseteq N_{\rho}(\tilde{G})$, we can see that by paying a negligible price in the robustness and correlation guarantees, we can use the blowing-up lemma to boost the probability of success of the algorithm to $1-o(1)$. 

It is worth noting that the boosting argument can give us exponentially high probability and not only $1-o(1)$. Furthermore, the argument is not unique to the stochastic block model and can be applied to a wide range of estimation problems.

==> content/robustness.tex <==
\section{Robustness}\label{sec:robustness}

\Tnote{This section should be formally correct but the exposition needs to be improved. A bit less than a day of work should be enough to fix it.}

\newcommand{\neighborhood}[1]{\Paren{100\cdot s\log s\cdot d \cdot \log^{#1}n}}
\newcommand{\specialneighborhood}{\Paren{100e\cdot s\log s\cdot d}}
\newcommand{\denominator}[1]{\Paren{100\cdot s\log s\cdot \log^{#1}n}}
\newcommand{\boundq}[2]{{#2\Paren{100\cdot s\log s\cdot d^2 \cdot \log^{#1}n}}}
\newcommand{\specialboundq}[1]{{#1\Paren{100e\cdot s\log s\cdot d^2}}}

Scheme:
\begin{enumerate}
	\item the adversary modifies the graph.
	\item for all the columns that violates the bound we remove all edges of the corresponding vertex.
	\item at most a constant fraction $2\rho(n)$ of the vertices can violate the bound. 
	\item the total number of edges of such fraction is at most $C\cdot \rho(n)d^{O(s)}$ for some universal constant $C$\todo.
	\item thus we may assume that at each step to go from $G$ to $G'$ we are not violating the bounds.
\end{enumerate}

We prove here that for random graphs,  single edge additions or deletions do not significantly change the value of the polynomial $Q^s(X)$.

 \begin{definition}\label{def:family_graph_distribution}
	Let $[n]$ be a set of vertices. And let $p\in \Brac{0,1}^{\binom{n}{2}}$ be a vector index by sets $\Set{i,j}$ with $i,j \in [n]$.
	Then consider the distribution $D_p$ where $G\sim D_p$ is obtained sampling independently each edge $i,j$ with probability $p_{i,j}$
	%We consider distributions over graphs on $n$ vertices such that each edge $e$ is sampled independently with probability $d_e$, where for each edge $e$, the value $d_e$ is a fixed  parameter of the distribution.
	We let $d$ be such that
\end{definition}

Notice that the null distribution of \cref{problem:planted-version} satisfy \cref{def:family_graph_distribution} with parameter $d$ for all edges.

Notice that we can work with such family of distribution since the properties we will study --namely the size of the $s$-neighborhood and the existence of cycles-- are increasing properties of random graphs (see \todo). 


%\Tnote{We can use such family because size of neighborhoods and number of cycles are increasing properties. Prove a lemma}

So, observe that the \Erdos \Renyi distribution satisfies \cref{def:family_graph_distribution}, similarly also the marginal distribution $\plantedd (\cdot, Y)$ as introduced in \cref{problem:planted-version} satisfies \cref{def:family_graph_distribution} with parameter $p=(1+\eps/2)d$.

The main result of the section is the theorem below.

\begin{theorem}\label{thm:robustness_technical}
	Let $G$ be a graph on $n$ vertices sampled from a distribution $D$ satisfying \cref{def:family_graph_distribution} with parameter $d>0$. Let $s>e$\Tnote{Check s,d dependency, maybe s>d?} be an integer and suppose $n\geq 10 s \log (s\cdot d \cdot 10)$.  Consider a non-negative function $\rho:\N \rightarrow \N_{\geq 0}$.
	Let $G'$ be a graph obtained from $G$ applying $\rho(n)$ arbitrary edge edits \Tnote{Better phrasing?}. Then, for any matrix $A\in \R^{n\times n}$ with $\Normi{A}=1$,
	\begin{align*}
	%	\Abs{\iprod{Q(X_G)-Q(X_{G'}), A}}\lesssim \rho n \cdot \specialboundq{O(s\cdot n)}^{3s}\,.
	\Abs{\iprod{Q(X_G)-Q(X_{G'}), A}}\lesssim \rho( n) \cdot  n\cdot (s\cdot d)^{6s}
	\end{align*}
	with probability at least $0.99$.
\end{theorem}

Our strategy will be the following. Suppose that we remove (or add) a single edge $ij\in E(G)$. So that $G'=G-ij$. Then, first we prove that for vertices $a,b$ far from both $i$ and $j$, the polynomial $q_{a,b}(X_{G'})$ is very close to $q_{a,b}(X_G)$.  Second we will show that even though for close vertices the change is more significant, such vertices are too few to significantly alter the spectrum of $Q(X_G)$.

We will further split our analysis between the case in which some vertex in $\Set{a,b,i,j}$ is in a cycle and the case in which the graph looks like an infinite tree to the eyes of the vertices $a,b,i,j$.
The following lemma captures this reasoning.

\begin{lemma}\label{lem:polynomial_change}
	Let $G$ be a graph sampled from a distribution $D$ satisfying \cref{def:family_graph_distribution} with parameter $d > 0$. Let $s>0$ be an integer. Let $i,j,a,b \in V(G)$ be vertices satisfying $\max_{v\in \Set{a,b,i,j}}\Card{N^{\ell}(v)}\leq (d\cdot q)^{\ell}$ for some $q\geq 100e\cdot s\log s$ and for all $\ell \in [s]$.
%	\begin{itemize}
	%	\item $\max_{v\in \Set{a,b,i,j}}\Card{N^{s}(v)}\leq (d\cdot q)^{s}$ for some $q>0\,.$
	%	\item  either $\Set{i,j} \cap N^s(a)=\emptyset$ or $\Set{i,j} \cap N^s(b)=\emptyset$. \Tnote{to split further in the case whether both a,b are far or only one of the two is far}
%	\end{itemize} 
	Suppose $\ij \in E(G)$, and consider the graph $G'=G-\ij$. Then the following bounds hold.
	{
	\newcommand{\differenceForOneEdit}[1]{s\Paren{2d^2\cdot q}^{#1}}
	\begin{enumerate}
		\item Suppose there is non cycle $C$ of length $\leq s$ in $G$ such that $\Set{a,b,i,j}\cap V(C)\neq \emptyset$.
		\begin{enumerate}
			\item \label{case:1a} If  $\Set{i,j} \cap N^s(a)=\emptyset$ and $\Set{i,j} \cap N^s(b)=\emptyset$, then
				\begin{align*}
						\Abs{q_{ab}(X_{G'}) -q_{ab}(X_G)}\lesssim \differenceForOneEdit{s} \cdot n^{-1}%\lesssim 2(d\cdot q)^{s}\cdot n^{-2}\,.
				\end{align*}
			\item \label{case:1b}If either $\Set{i,j} \cap N^s(a)=\emptyset$ or $\Set{i,j} \cap N^s(b)=\emptyset$, then
				\begin{align*}
					\Abs{q_{ab}(X_{G'}) -q_{ab}(X_G)}\lesssim \differenceForOneEdit{s}  %\lesssim 2(d\cdot q)^{s}\cdot n^{-1}\,.
				\end{align*}
			\item \label{case:1c}If $\Set{i,j}\cap N^s(a)\neq \emptyset$ and $\Set{i,j}\cap N^s(b)\neq \emptyset$, then 
			\begin{align*}
				\Abs{q_{ab}(X_{G'}) -q_{ab}(X_G)}\lesssim \differenceForOneEdit{s}  \cdot n%\lesssim 2(d\cdot q)^{s}\,.
			\end{align*}
		\end{enumerate}
	%	\begin{align*}
		%	\Abs{q_{ab}(X_{G'}) -q_{ab}(X_G)}\lesssim 2(d\cdot q)^{s}\cdot n^{-1}\,,
	%	\end{align*}
	\item Otherwise,
	\begin{enumerate}
		\item \label{case:2a}If  $\Set{i,j} \cap N^s(a)=\emptyset$ and $\Set{i,j} \cap N^s(b)=\emptyset$, then
		\begin{align*}
			\Abs{q_{ab}(X_{G'}) -q_{ab}(X_G)}\lesssim\differenceForOneEdit{s^2} \cdot n^{-1}\,.
		\end{align*}
		\item \label{case:2b}If either $\Set{i,j} \cap N^s(a)=\emptyset$ or $\Set{i,j} \cap N^s(b)=\emptyset$, then
		\begin{align*}
			\Abs{q_{ab}(X_{G'}) -q_{ab}(X_G)}\lesssim \differenceForOneEdit{s^2} \,.
		\end{align*}
		\item \label{case:2c}If $\Set{i,j}\cap N^s(a)\neq \emptyset$ and $\Set{i,j}\cap N^s(b)\neq \emptyset$, then 
		\begin{align*}
			\Abs{q_{ab}(X_{G'}) -q_{ab}(X_G)}\lesssim \differenceForOneEdit{s^2}  \cdot n\,.
		\end{align*}
	%\begin{align*}
		%\Abs{q_{ab}(X_{G'}) -q_{ab}(X_G)}\lesssim 2(d\cdot q)^{s^2}\cdot n^{-1}\,.
	%\end{align*}
	\end{enumerate}
	\end{enumerate}
	%obtained as follows
	%\begin{align*}
	%	G' := \begin{cases}
	%		G+ \ij&\text{ if }\ij \notin E(G)\\
	%		G - \ij& \text{ if } \ij \in E(G)\,.
	%	\end{cases}
	%\end{align*}
	%Suppose that \Tnote{Good event happens}
	}
\end{lemma}

We prove  \cref{lem:polynomial_change} in \cref{sec:robustness_proof_polynomial_change} and use it here to  to obtain \cref{thm:robustness_technical}.



\begin{proof}[Proof \cref{thm:robustness_technical}]
	For $i \in \Brac{\lceil \log \log n\rceil -1}$, define the sets
	\begin{align*}
		N^{i,s}(G)&:=\Set{v \in V(G)\suchthat \neighborhood{1/i}^s \leq \Card{N^s(v)}\leq \neighborhood{2/i}^s}\,.
		%P^{i}(G)&:= \Set{q_{ab}(X_G)\suchthat   \Set{a,b}\cap N^{i,s}(G)\neq \emptyset \text{ and for all $j > i$, }  \Set{a,b}\cap N^{j,s}(G)= \emptyset }\,.
	\end{align*} 
	For $i=\lceil \log \log n\rceil$, instead define
	\begin{align*}
		N^{i,s}(G)&:=\Set{v \in V(G)\suchthat \Card{N^s(v)}\leq \Paren{100\cdot s\log s\cdot d }^s}\,,
	\end{align*}
	and finally for each $i \in \Brac{\lceil \log \log n\rceil}$ let
	\begin{align*}
		P^{i}(G)&:= \Set{q_{ab}(X_G)\suchthat   \Set{a,b}\cap N^{i,s}(G)\neq \emptyset \text{ and for all $j > i$, }  \Set{a,b}\cap N^{j,s}(G)= \emptyset }\,.
	\end{align*}
	We condition our analysis on the event that for all $i \in \Brac{\lceil \log \log n\rceil-1}$ the set $N^{i,s}(G)$ has cardinality at most $\frac{n}{\denominator{1/i}^{10s}}$.
	Furthermore we also condition the analysis on the event that at most $1000\cdot s^2 \cdot (e\cdot d)^s$ vertices in $G$ are part of a cycle of length $\leq s$. By \cref{lem:vertices_with_large_neighborhoods_are_few} (setting $\delta = 10s$) and  \cref{cor:existence_of_cycle_with_v} the intersection of these events has probability at least $0.998$. Notice also that by \cref{lem:bound_size_neighborhood} with high probability no vertex has $s$-neighborhood larger than $\Paren{10\cdot s\log s \cdot d \log n}^s$.
	
	Now, without loss of generality we may assume that $G'$ is obtained from $G$ by a sequence $E = \Set{e_1,\ldots,e_{\rho\cdot n}}$  of edge deletions, that is
	\begin{align*}
		G' = G - \sum_{e_i \in E} e_i \,.
	\end{align*}
	Let $V(E)\subseteq V(G)$ be the set of vertices in $G$ incident to the edges in $E$.
	For each $\alpha \in [\rho( n)]$, consider the graph $G_\alpha=G-\sum_{\beta \leq \alpha}e_\beta$ and let $G_0=G$. For each set $N^{i,s}$, also let $E^{i,s}:=N^{i,s}\cap V(E)$. Then
	\Tnote{Here we can improve the bound by counting the number of non-zero entries of $A$}
	\begin{align}
		\Abs{\iprod{Q(X_{G}) -Q(X_{G'}), A } }&\leq \underset{a,b \in [n]}{\sum}\Abs{q_{ab}(X_G)-q_{ab}(X_{G'})}\\
		&\leq \underset{\alpha \in [\rho(  n)]}{\sum}\underset{a,b \in [n]}{\sum}\Abs{q_{ab}(X_{G_\alpha})-q_{ab}(X_{G_{\alpha-1}})}\\
		%&\leq \underset{\alpha \in [\rho]}{\sum}\quad\underset{i \in \lceil\log\log n \rceil}{\sum} \quad\underset{q_{ab}\in P^i}{\sum}\Abs{q_{ab}(X_{G_\alpha})-q_{ab}(X_{G_{\alpha-1}})}\\
		&\leq \underset{i \in \lceil\log\log n \rceil}{\sum} \quad \underset{e_\alpha \in E^{i,s}}{\sum}\quad\underset{j  \in \Brac{\lceil\log\log n \rceil} }{\sum }\quad \underset{q_{ab}\in P^j}{\sum}\Abs{q_{ab}(X_{G_\alpha})-q_{ab}(X_{G_{\alpha-1}})} \label{eq:sum_q_entries}\,.
	\end{align}
	We  upper bound  the contribution of  elements in \cref{eq:sum_q_entries}.
	Consider $e_\alpha\in E^{i,s}$ with endpoints $u,v$, for some $i \in \Brac{\lceil \log \log n\rceil -1}$. Suppose first that no cycle in $G$ of length at most $s$ contains a vertex from $N^s(u)\cup N^s(v)$. 
	We bound 
	\begin{align}\label{eq:robustness_bound_single_edge}
		\underset{j  \in \Brac{\lceil\log\log n \rceil} }{\sum }\quad \underset{q_{ab}\in P^j}{\sum}\Abs{q_{ab}(X_{G_\alpha})-q_{ab}(X_{G_{\alpha-1}})}\,.
	\end{align}
	Before applying  \cref{lem:polynomial_change}  we count the occurrences of different types of pairs $(a,b)$ with $a,b\in V(G)$ applying \cref{lem:vertices_with_large_neighborhoods_are_few}.  
	\begin{itemize}
		\item For each $j\in \Brac{\lceil\log\log n \rceil -1}$, there are at most $\frac{2n^2}{\denominator{1/j}^{10s}}$ elements of the form \cref{case:1a} in \cref{eq:robustness_bound_single_edge}. For $j = \lceil \log\log n \rceil$ there are at most $n^2$. %for $j =\lceil\log\log n \rceil$ at most $n^2$.
		\item There are at most  $2\neighborhood{2/i}^s n$ elements of the form \cref{case:1b}  in \cref{eq:robustness_bound_single_edge}.
		\item There are at most $2\neighborhood{2/i}^{2s}$ elements of the form \cref{case:1c} in \cref{eq:robustness_bound_single_edge}.
		\item There are at most $2\cdot 10^6\cdot s^4 \cdot (e\cdot d)^{2s} + 2n\cdot 1000\cdot s^2 \cdot (e\cdot d)^s$ elements of the form \cref{case:2a} in \cref{eq:robustness_bound_single_edge}.
		\item There are at most $1000\cdot s^2 \cdot (e\cdot d)^s\cdot 2\neighborhood{2/i}^s$ elements of the form \cref{case:2b} in \cref{eq:robustness_bound_single_edge}.
		%\item There are at most $2\cdot 10^6\cdot s^6 \cdot (e\cdot d)^{2s}$ elements of the form \cref{case:2c} in \cref{eq:robustness_bound_single_edge}.
	\end{itemize}
	 
	 Applying \cref{lem:polynomial_change} we get an upper bound of $\boundq{2/i}{O(s\cdot n)}^{3s} $ on \cref{eq:robustness_bound_single_edge}. Similarly for $i=\lceil \log\log n \rceil$ we get an upper bound of $O(s\cdot n)\Paren{100\cdot s\log s \cdot d^2}^{3s}$.
	 
	Conversely suppose there exists a cycle of length at most $s$ containing either $u$ or $v$. The following bounds change.
	\begin{itemize}
		\item  For each $j\in \Brac{\lceil\log\log n \rceil -1}$, there are at most $\frac{2n^2}{\denominator{1/j}^{10s}}$ elements of the form \cref{case:2a} in \cref{eq:robustness_bound_single_edge}. For $j = \lceil \log\log n \rceil$ there are at most $n^2$. 
		\item There are at most $2n\cdot \neighborhood{2/i}^s$ elements of the form \cref{case:2b} in \cref{eq:robustness_bound_single_edge}.
		\item There are at most $2\neighborhood{2/i}^{2s}$ elements of the form \cref{case:2b} in \cref{eq:robustness_bound_single_edge}.
	\end{itemize}
	
	Applying \cref{lem:polynomial_change} we get that  an upper bound of $\boundq{2/i}{O(s\cdot n)}^{s^2+3s}$ on \cref{eq:robustness_bound_single_edge}. Similarly for $i=\lceil \log\log n \rceil$ we get an upper bound of $O(s\cdot n)\Paren{100\cdot s\log s \cdot d}^{s^2+3s}$.
	
	There are at most $ 2\neighborhood{}^s\cdot 1000\cdot s^2 \cdot (e\cdot d)^s$ vertices in $V(E)$ at distance at most $s$ from a cycle of length $s$. 
	Moreover, by our conditioning for $i \in\Brac{\lceil \log\log n \rceil -1}$ we have $\Card{V(E^{i,s})} \leq  \frac{2n}{\denominator{1/i}^{10s}}$ and finally we have we have $\Card{V(E)} \leq 2\rho n$.
	
	Putting everything together
	\begin{align*}
		\Abs{\iprod{Q(X_{G}) -Q(X_{G'}), A } }&\leq \underset{a,b \in [n]}{\sum}\Abs{q_{ab}(X_G)-q_{ab}(X_{G'})}\\
		&\leq\underset{i \in \lceil\log\log n \rceil}{\sum} \quad \underset{e_\alpha \in E^{i,s}}{\sum}\quad\underset{j  \in \Brac{\lceil\log\log n \rceil} }{\sum }\quad \underset{q_{ab}\in P^j}{\sum}\Abs{q_{ab}(X_{G_\alpha})-q_{ab}(X_{G_{\alpha-1}})}\\
		&\lesssim \rho n \cdot  \specialboundq{O(s\cdot n)}^{3s}\,.
	\end{align*}
	
	\iffalse
	
	
	there exists a cycle of length at most $s$ containing either $u$ or $v$.
	
	
	Conversely, if 
	Then for each $j \leq \Brac{\lceil \log \log n\rceil-1} $,
	we get by \cref{lem:polynomial_change} 
	\begin{align*}
		\underset{q_{ab}\in P^j}{\sum}\Abs{q_{ab}(X_{G_\alpha})-q_{ab}(X_{G_{\alpha-1}})}
		% \leq& 2n \cdot \frac{n}{\Paren{10s\cdot \log s\cdot \log^{1/j}n}^{2s}}\cdot \Paren{10s\cdot \log s\cdot \log^{2/i}n}^s\cdot n^{-2} \\
		%+&  2\Paren{10s\cdot \log s\cdot \log^{2/j}n}^{s} \cdot \frac{n \cdot \Paren{10s\cdot \log s\cdot \log^{2/i}n}^{s}}{\Paren{10s\cdot \log s\cdot \log^{1/j}n}^{2s}}\cdot   n^{-	1}\\
		%+& 2 \Paren{10s\cdot \log s\cdot \log^{2/i}n}^{3s}\\
		\lesssim& \frac{\Paren{10\cdot s\log s\cdot d\cdot \log^{2/i}n}^{3s}}{ \Paren{10\cdot s\log s\cdot d\cdot \log^{2/j}n}^{3s}}\,,
	\end{align*}
	Since in such sum we have at most $n\cdot  \frac{n}{\Paren{10s\cdot \log s\cdot \log^{1/j}n}^{2s}}$ element of the form \cref{case:1a}, at most $\frac{n}{\Paren{10s\cdot \log s\cdot \log^{1/j}n}^{2s}}$ elements of the form \cref{case:1b} and most $\Paren{10s\cdot \log s\cdot \log^{1/i}n}^{2s}$ elements of the form \cref{case:1c}.  Moreover we have at most  $\frac{n\cdot \Paren{10s\cdot \log s\cdot \log^{1/j}n}^{s}}{\Paren{10s\cdot \log s\cdot \log^{1/j}n}^{2s}}$ element of the form \cref{case:2a}.
		
	Suppose now that there exists $w\in N^s(u)\cup N^s(v)$ that is part of a cycle of length at most $s$ in $G$.
	Then by \cref{lem:polynomial_change} and a similar counting argument \Tnote{Write the argument?}
	\begin{align*}
			\underset{q_{ab}\in P^j}{\sum}\Abs{q_{ab}(X_{G_\alpha})-q_{ab}(X_{G_{\alpha-1}})}\lesssim& \Paren{10\cdot s\log s\cdot d\cdot \log^{2/i}n}^{3s^2}\,.
	\end{align*}
	Now $\Card{E^{i,s}}\leq \Card{N^{i,s}}\cdot \Paren{10\cdot s\log s\cdot d\cdot \log^{2/i}n}^{s}$ and at most $1000\cdot s^3 \cdot (e\cdot d)^s\cdot \Paren{d\cdot \log n}^s $ any of them are at distance at most $s$ from a cycle of length $\leq s$. Thus
	\begin{align*}
		\underset{e_\alpha \in E^{i,s}}{\sum}\quad\underset{j  \in \Brac{\lceil\log\log n \rceil} }{\sum }\quad \underset{q_{ab}\in P^j}{\sum}\Abs{q_{ab}(X_{G_\alpha})-q_{ab}(X_{G_{\alpha-1}})} &\leq  O(d)^{4s}\cdot n\,.
	\end{align*}
	
	
	
	

	
	 for each fixed $i$.
	
	

	 and additonally for all $i \in \Brac{\lceil \log \log n\rceil}$ define the set. Then for each edge $e\in E^{i,s}$
	
	
	 we have at most $\frac{2n^2}{\Paren{10s\cdot \log s\cdot \log^{1/i}n}^{2s}}$    $\Card{N^{i,\ell}\cap E}\leq \min \Set{\rho n, }$
	For each edge $e_i \in E$, there are at most 
$100\cdot s^3\cdot (e\cdot d)^s$ edges in $E_1$ \cref{eq:sum_q_entries}
	There are at most 

	
	Now, let $E_1 = \Set{e_1,\ldots,e_\rho}$ be the sete of edge additions and $E_2=\Set{e'_1,\ldots,e'_{\rho'}}$ the set of deletions applied to $G$ so that 
	\begin{align*}
		G' = G +\sum_{i\in [\rho]} e_i - \sum_{j \in [\rho']}e'_j\,.
	\end{align*}
	Also define $G_1 = G +\sum_{i\in [\rho]} e_i$ and $G_2 = G_1- \sum_{j \in [\rho']}e'_j\,.$
	We show that 
	\begin{align*}
		\Abs{\iprod{Q(X_{G}) -Q(X_{G_1}), A } }\leq \todo\,.
	\end{align*}
	The same proof applies to $	\Abs{\iprod{Q(X_{G_2}) -Q(X_{G_1}), A } }$, then putting the two together we obtain \cref{thm:robustness_technical}.
	So first observe that,
	\begin{align*}
		\Abs{\iprod{Q(X_{G}) -Q(X_{G_1}), A } }&\leq \underset{a,b \in [n]}{\sum}\Abs{q_{ab}(X_G)-q_{ab}(X_{G_1})}\\
		&\leq \underset{v \in [\rho]}{\sum}\underset{a,b \in [n]}{\sum}\Abs{q_{ab}(X_{G+})-q_{ab}(X_{G_1})}\,.
	\end{align*}
	Now, there are at most $100\cdot s^3\cdot (e\cdot d)^s$ edges in $E_1$ that are part of a cycle of length at most $s$.
	
	
	Now, under these conditions it suffices to show that for a single edge delition/addition the bound
	\begin{align*}
		\Abs{\iprod{Q(X_G)-Q(X_{G'}), A}}\leq \todo 
	\end{align*}
	holds. Then simply repeating the reasoning for each edge addition and deletion we will prove the theorem.
	So without loss of generality consider the graph $G'=G-\ij$ for some arbitrary edge $\ij \in E(G)$.
	 \fi
\end{proof}









\subsection{Proof of \cref{lem:polynomial_change}}\label{sec:robustness_proof_polynomial_change}

In order to prove \cref{lem:polynomial_change}, we introduce some notation first. Let $G$ be a graph on $n$ vertices and fixed vertices $i,j \in V(G)$. For $a,b \in V(G)$, we define  the set $\cW:=\Set{S\in \saw{ab}{s}(K_n)\suchthat \ij \in E(S)}$ and the sets $\cW_0(G),\ldots, \cW_s(G)$ where $\cW_\ell(G) := \Set{S\in \cW \suchthat \Card{E(S)\setminus E(G)} = \ell }$, that is $\cW_\ell(G)$ contains the set of self-avoiding walks over $K_n$ which go through edge $\ij\in E(K_n)$ and   have exactly $\ell$ edges not in $E(G)$.  Recall also that for a walk $S$ of length $\ell$, we denote its sequence of edges by $e_1,\ldots,e_\ell$.\Tnote{Add to notation}.

To prove \cref{lem:polynomial_change} we start by showing  that the number of vertices with many self-avoiding walk of length $\leq s$ decays fast. 

\begin{lemma}\label{lem:bound_number_of_patterns_random_graph}
	Let $G$ be a graph on $n$ vertices sampled from a distribution $D$ satisfying \cref{def:family_graph_distribution} with parameter $d > 0$.  Let $s>0$ be an integer. 
	Suppose $\log n \gtrsim s^2\log (s\cdot d\cdot \log n)$.
	For $i \in \Brac{\lceil \log \log n\rceil -1}$ and $\ell \in [s]$, define the set
	\begin{align*}
		N^{i,\ell}(G):=\Set{v \in V(G)\suchthat \neighborhood{1/i}^\ell \leq \Card{N^\ell(v)}\leq \neighborhood{2/i}^\ell}\,.%\Paren{10\cdot s\log s\cdot d \cdot \log^{2/i}n}^\ell}\,.
	\end{align*} 
	Then with probability at least $0.998$, for all $i \in \Brac{\lceil \log \log n\rceil}$ and all $\ell \in [s]$
	\begin{align*}
		\Card{N^{i,\ell}(G)}\cdot \Card{\underset{v \in V(G)}{\bigcup} \saw{v}{\ell}(G)} \leq 2n \cdot d^\ell\,.
	\end{align*}
	Moreover, for $i =\lceil \log\log n \rceil$ let $N^{i,\ell}(G):=\Set{v \in V(G)\suchthat \Card{N^\ell (v)}\leq \specialneighborhood ?? \ell }$.\Dnote{FIXME: there was a latex error here} Then %\Paren{10\cdot s\log s\cdot d }^\ell }$. Then
	\begin{align*}
		\Card{N^{i,\ell}(G)}\cdot \Card{\underset{v \in V(G)}{\bigcup} \saw{v}{\ell}(G)} \leq \specialneighborhood^\ell\cdot n\,.
	\end{align*}
	\begin{proof}
		We condition our analysis on the event thatthere are at most $1000\cdot s^2 \cdot (e\cdot d)^\ell$ vertices that are parts of a cycle of length $\leq s$ in $G$. By \cref{cor:existence_of_cycle_with_v} such event holds with probability at least $0.999$.
		Next, applying \cref{lem:vertices_with_large_neighborhoods_are_few} with $\delta=\max\Set{4s,10}$ we have that with probability at least $0.999$
		for all  $i \in \Brac{\lceil \log \log n\rceil}$ and all $\ell \in [s]$, the set $N^{i,\ell}(G)$
		%\begin{align*}
		%	N^{i,\ell}(G):=\Set{v \in V(G)\suchthat 100\cdot \log s\cdot d^\ell \cdot \log^{1/i}n\leq \Card{N^\ell(v)}\leq 100\cdot \log s\cdot d^\ell \cdot \log^{2/i}n}\,,
		%	\end{align*} 
		has cardinality at most $\frac{n}{\Paren{10s\cdot \log s\cdot \log^{1/i}n}^{2s}}$.
		%Among the vertices in $N^{i,\ell}(G)$, at most $1000\cdot s^2 \cdot (e\cdot d)^\ell$ of them are part of a cycle of length $\leq \ell$.  
		Applying \cref{fact:bound_saw_from_v} we get that
		\begin{align*}
			\Card{N^{i,\ell}(G)}\cdot \Card{\underset{v \in V(G)}{\bigcup} \saw{v}{\ell}(G)} \leq& \frac{n}{\denominator{1/i}^{10s}}\neighborhood{2/i}^\ell \\&+ 1000\cdot s^2 \cdot (e\cdot d)^\ell \cdot\neighborhood{2/i}^{s\cdot \ell}\\
			&\leq 2n \cdot d^\ell\,.
		\end{align*}
		\Tnote{Notice that the bound above coudl be improved to $n$.}
		%\begin{align*}
		%	\Card{N^{i,\ell}(G)}\cdot \Card{\underset{v \in V(G)}{\bigcup} \saw{v}{\ell}(G)} \leq& \frac{n}{\Paren{10s\cdot \log s \cdot \log^{1/i} n}^{2s}} \Paren{10\cdot s\log s\cdot d \cdot \log^{2/i}n}^\ell \\&+ 1000\cdot s^2 \cdot (e\cdot d)^\ell \cdot \Paren{10\cdot \log s\cdot d \cdot \log^{2/i}n}^{s\cdot \ell}\\
		%	&\leq 2n \cdot d^\ell\,.
	%	\end{align*}
		The bound on $N^{*,\ell}$ for $i=\lceil\log\log n\rceil$ follows directly observing that there are $n$ vertices in $G$ and at most   $1000\cdot s^2 \cdot (e\cdot d)^\ell$ of them are part of a cycle of length $\leq \ell$.  
	\end{proof}
\end{lemma}

Next, we bound the cardinality of $\cW_\ell$ depending on the distance between the vertices $a,b,i,j$ in $G$.

\begin{lemma}\label{lem:bound_w_change}
	With the same settings as \cref{lem:polynomial_change}, for any $\ell\leq s$, the following bounds hold.
	\begin{enumerate}
		\item Suppose there is non cycle of length $\leq s$ in $G$ such that $\Set{a,b,i,j}\cap V(C)\neq \emptyset$, then 
		\begin{enumerate}
			\item \label{case:w1a}If $\Set{i,j}\cap N^s(a)=\emptyset$ and $\Set{i,j}\cap N^s(b)=\emptyset$ then
			\begin{align*}
				\Card{\cW_\ell(G)}\leq ( 2 d \cdot q)^{s}\cdot n^{\ell-2}\,.
			\end{align*}
			\item \label{case:w1b}If either $\Set{i,j}\cap N^s(a)=\emptyset$ or $\Set{i,j}\cap N^s(b)=\emptyset$ then
				\begin{align*}
				\Card{\cW_\ell(G)}\leq ( 2 d \cdot q)^{s}\cdot n^{\ell-1}\,.
			\end{align*}
			\item \label{case:w1c}If $\Set{i,j}\cap N^s(a)\neq \emptyset$ and $\Set{i,j}\cap N^s(b)\neq \emptyset$ then
			\begin{align*}
				\Card{\cW_\ell(G)}\leq ( 2 d \cdot q)^{s}\cdot n^{\ell}\,.
			\end{align*}
		\end{enumerate}
		\item Otherwise,
		\begin{enumerate}
			\item \label{case:w2a}If $\Set{i,j}\cap N^s(a)=\emptyset$ and $\Set{i,j}\cap N^s(b)=\emptyset$ then
			\begin{align*}
				\Card{\cW_\ell(G)}\leq ( 2 d \cdot q)^{s^2}\cdot n^{\ell-2}\,.
			\end{align*}
			\item \label{case:w2b}If either $\Set{i,j}\cap N^s(a)=\emptyset$ or $\Set{i,j}\cap N^s(b)=\emptyset$ then
			\begin{align*}
				\Card{\cW_\ell(G)}\leq ( 2 d \cdot q)^{s^2}\cdot n^{\ell-1}\,.
			\end{align*}
			\item \label{case:w2c}If $\Set{i,j}\cap N^s(a)\neq \emptyset$ and $\Set{i,j}\cap N^s(b)\neq \emptyset$ then
			\begin{align*}
				\Card{\cW_\ell(G)}\leq ( 2 d \cdot q)^{s^2}\cdot n^{\ell}\,.
			\end{align*}
		\end{enumerate} 
		%\tochange
		%\begin{align*}
		%	\Card{\cW_\ell(G)}\leq ( 2 d \cdot q)^{s}\cdot n^{\ell-1}\,,
		%\end{align*}
		%\item otherwise 
		%\begin{align*}
		%	\Card{\cW_\ell(G)}\leq ( 2d \cdot q)^{s^2}\cdot n^{\ell-1}\,.
		%\end{align*}
	\end{enumerate}
	\begin{proof}
		We further decompose $\cW_\ell(G)$ into the following subsets: fix $\gamma\leq s$ and indices $\alpha_1< \ldots<\alpha_\ell$. Then 
		\begin{align*}
			\cS_{\gamma,\alpha_1,\ldots.\alpha_\ell}:= \Set{S \in \cW_\ell(G)\suchthat  \ij \text{ is the $\gamma$-th edge $e_\gamma$ in $S$ and }  \forall t \in [\ell], e_{\alpha_t}\notin E(G) }\,.
		\end{align*}
		In other words, we look at the subsets of self-avoiding walks over $K_n$ in which $\ij$ is in a given position and a fixed subset of edges of the walk do not appear in $G$.
		
		We start by proving \cref{case:w1a}. Other cases will be similar.
		In the settings of \cref{case:w1a}, we have $\alpha_1<\gamma$ and $\alpha_\ell> \gamma$.
		Since by assumption $\Card{N^{\alpha_1-1}_G(a)}\leq (d\cdot q)^{\alpha_1-1}$, by \cref{fact:bound_saw_from_v} there are at most $(d\cdot q)^{\alpha_1 -1}$ different patterns for the first $\alpha_1 -1$ edges. Similarly, we have at most $\Paren{d\cdot q}^{s-\alpha_\ell}$ for the last $s-\alpha_\ell$ edges.
		
		So let $\alpha_p$ be the largest index in  $\Set{\alpha_1,\ldots,\alpha_\ell}$ smaller than $\gamma$,
		then by assumption on the size of the $s$-neighborhood of $i$ and $j$, we have at most $(d\cdot q)^{\alpha_p-\gamma-1}$ patterns for $e_{\alpha_p},\ldots,e_{\gamma-1}$ as it must be that $e_{\alpha_p}$ is incident to some vertex in $N_G^{\alpha_p-\gamma-1}(i)$. Similarly we have at most $(d\cdot q)^{\alpha_\gamma-\alpha_{p+1}}$ patterns for $e_{\gamma},\ldots,e_{\alpha_{p+1}-1}$.
		
		Next let $t\in [\ell-1]$, $t\neq p$. We bound the number of patterns for edges $e_{\alpha_t},\ldots,e_{\alpha_{t+1}-1}$. To this end let $z = \alpha_t -\alpha_{t+1}-1$, that is the number of edges in $e_{\alpha_t},\ldots,e_{\alpha_{t+1}-1}$.
		
		By \cref{lem:bound_number_of_patterns_random_graph} we have at most $2n\cdot\Paren{100e\cdot s\log s \cdot d}^z$ distinct patterns for the edges $e_{\alpha_t},\ldots,e_{\alpha_{t+1}-1}$.
		
		Combining all the possible patterns for each subwalk  $e_{\alpha_t},\ldots,e_{\alpha_{t+1}-1}$ we get that 
		\begin{align*}
			\Card{\cS_{\gamma,\alpha_1,\ldots.\alpha_\ell}}\leq n^{\ell-2}\cdot\max\Set{ \Paren{d\cdot q}^{s}, (10\cdot s \log s \cdot d)^s}\,.
		\end{align*} \Tnote{That is why we forced $q$ to be larger than $s\log s \cdot 10$}
		For \cref{case:w1b} the analysis is analogous with the exception that we are only guaranteed that one between $a_1 < \gamma$ and $a_\ell > \gamma$ exists. Thus repeating the analysis we get
		\begin{align*}
			\Card{\cS_{\gamma,\alpha_1,\ldots.\alpha_\ell}}\leq n^{\ell-1}\cdot \Paren{d\cdot q}^{s}\,.
		\end{align*} 
		Similarly, for \cref{case:w1c} there might not be any $a_1 < \gamma$ and any  $a_\ell > \gamma$. So we can only prove that 
		\begin{align*}
			\Card{\cS_{\gamma,\alpha_1,\ldots.\alpha_\ell}}\leq n^{\ell}\cdot \Paren{d\cdot q}^{s}\,.
		\end{align*} 
	
		Now, for the cases \cref{case:w1a}, \cref{case:w1b} and \cref{case:w1c} the proof follows the same structure outlined above, with the crucial difference that we may have $(d\cdot q)^{s(\alpha_1-1)}$ distinct patterns for the first $\alpha_1-1$ edges, $(d\cdot q)^{s(\alpha_{p+1}-\alpha_{p}-1)}$ for the edges $e_{\alpha_p},\ldots,e_{\alpha_{p+1}-1}$ and finally $(d\cdot q)^{s(s-\alpha_\ell)}$ for the last $s-\alpha_\ell$ egdes. %$(d\cdot q)^{s(\gamma-1-\alpha_p)}$ for the edges $e_\alpha_p,\ldots,e_\gamma$, $(d\cdot q)^{s(\alpha_{p+1}-\gamma-1)}$ for the edges
		For each case considered, the claim follows observing that there are at most $\binom{s}{\ell}$ distinct $\cS_{\gamma,\alpha_1,\ldots.\alpha_\ell}$ and that
		$\cW_\ell(G) = \underset{\gamma,\alpha_1< \ldots<\alpha_\ell\in [s]}{\bigcup}\cS_{\gamma,\alpha_1,\ldots.\alpha_\ell}$.
	\end{proof}
\end{lemma}

We can now prove \cref{lem:polynomial_change}.

\begin{proof}[Proof of \cref{lem:polynomial_change}]
	\Tnote{This should be changed once we generalize the polynomial to $k\geq 2$}
	Recall that $q_{ab}(X_G) \leq (1+o(1))\cdot n \Paren{\frac{4}{\eps \cdot d}}^s\underset{S\in \saw{ab}{s}}{\sum}p_S(X_G) \leq  (1+o(1))n \Paren{\frac{4}{\eps \cdot d}}^s \underset{S\in \saw{ab}{s}}{\sum}\Paren{\frac{-d}{n}}^{\Card{E(S)\setminus E(G)}}\,.$ %\frac{n}{\Paren{\eps\cdot d}^s}\underset{S\in \saw{ab}{s}}{\sum}p_S(X_G) = (1\pm o_{\sqrt{n}}(1))\cdot  \frac{n}{\Paren{\eps\cdot d}^s}\underset{S\in \saw{ab}{s}}{\sum}\Paren{\frac{-d}{n}}^{\Card{E(S)\setminus E(G)}}\,.$
	We also have that 
	\begin{align*}
		\Abs{q_{ab}(X_{G'}) -q_{ab}(X_G)} &= (1\pm o(1))\cdot n \Paren{\frac{4}{\eps \cdot d}}^s\Abs{\underset{S\in \saw{ab}{s}}{\sum}p_S(X_G) - \underset{S\in \saw{ab}{s}}{\sum}p_S(X_{G'}) }\\
		%&\leq (1\pm o(1))\frac{n}{\Paren{\eps\cdot d}^s} \underset{\substack{S\in \saw{ab}{s}\\\text{s.t. } \ij \in E(S) }}{\sum} \Abs{p_S(X_G)} + \Abs{p_S(X_{G'})}\\
		%&\leq (1\pm o(1))\frac{n}{\Paren{\eps\cdot d}^s} \underset{\substack{S \in \cW_\ell\\ \ell \in [s]}}{\sum} \Abs{p_S(X_G)} + \Abs{p_S(X_{G'})}\,.
		&\leq  (1\pm o(1))\cdot n \Paren{\frac{4}{\eps \cdot d}}^s \underset{\substack{S\in \saw{ab}{s}\\\text{s.t. } \ij \in E(S) }}{\sum} \Abs{p_S(X_G)} + \Abs{p_S(X_{G'})}\\
		&\leq (1\pm o(1))\cdot n \Paren{\frac{4}{\eps \cdot d}}^s \underset{\substack{S \in \cW_\ell\\ \ell \in [s]}}{\sum} \Abs{p_S(X_G)} + \Abs{p_S(X_{G'})}\\
		&\leq (1\pm o(1))\cdot n \Paren{\frac{4}{\eps \cdot d}}^s \underset{\substack{S \in \cW_\ell\\ \ell \in [s]}}{\sum} 2\Paren{\frac{d}{n}}^\ell\,.
	\end{align*}
	Notice that for each $S\in \cW_\ell(G)$ we have $\Abs{p_S(X_G)}\leq\Paren{\frac{d}{n}}^\ell$ and similarly  for all $S' \in \cW_\ell(G')$, $\Abs{p_S(X_{G'})}\leq\Paren{\frac{d}{n}}^{\ell}$.
	We explicitly show how to prove \cref{case:1a}. Other cases follows by the same argument applying the corresponding case of \cref{lem:bound_w_change}.
	In the settings of \cref{case:1a}, we get
	\begin{align*}
		\Abs{q_{ab}(X_{G'}) -q_{ab}(X_G)} &\leq  (1\pm o(1))\cdot n \Paren{\frac{4}{\eps \cdot d}}^s \underset{\substack{S \in \cW_\ell\\ \ell \in [s]}}{\sum} \Abs{p_S(X_G)} + \Abs{p_S(X_{G'})}\\
		&\leq  (1\pm o(1))\cdot n \Paren{\frac{4}{\eps \cdot d}}^s \underset{\ell \in [s]}{\sum} 2\Paren{\frac{d}{n}}^{\ell}\cdot \Paren{2d\cdot q}^s\cdot n^{\ell-2}\\
		&\lesssim \frac{s\Paren{2d^2\cdot q}^{s}}{n}\,.
	\end{align*}
\end{proof}


